GANerated Hands for Real-time 3D Hand Tracking from Monocular RGB

We address the highly challenging problem of real-time 3D hand tracking based on a monocular RGB-only sequence. Our tracking method combines a convolutional neural network with a kinematic 3D hand model, such that it generalizes well to unseen data, is robust to occlusions and varying camera viewpoints, and leads to anatomically plausible as well as temporally smooth hand motions. For training our CNN we propose a novel approach for the synthetic generation of training data that is based on a geometrically consistent image-to-image translation network. To be more specific, we use a neural network that translates synthetic images to "real" images, such that the so-generated images follow the same statistical distribution as real-world hand images. For training this translation network we combine an adversarial loss and a cycle-consistency loss with a geometric consistency loss in order to preserve geometric properties (such as hand pose) during translation. We demonstrate that our hand tracking system outperforms the current state-of-the-art on challenging RGB-only footage.

==> overview.tex <==
\section{Overview}
\label{sec:overview}
%

%To achieve our hand tracking system we tackle three main tasks. First, we generate training data (Sec.~\ref{sec:GAN_for_training}, and Fig.~\ref{fig:trainingPipeline}, left), which we use to train a neural network for 2D and 3D hand joint localization, and Fig.~\ref{fig:trainingPipeline}, right). Subsequently, to perform hand tracking we use the JORNet to predict joint locations that are eventually fed into a kinematic hand skeleton fitting method .



% \franzi{Real-time system similar to ICCV paper: live RGB-only video stream is fed to CNN pose regressor to estimate 2D heatmaps and 3D pose of 21 keypoints of the hand. Here, the 3D pose is root relative and normalized s.t. dist(wrist, middle MCP joint) = 1.
% Afterwards, the global position is computed based on heatmaps, intrinsic camera parameters, and skeleton size (either known or mean, relative bone lengths from CNN). The final pose is refined by minimizing an energy function which consists of 2D IK, 3D IK, temporal smoothness, joint limits.}


